Games with Costs and Delays

We demonstrate the usefulness of adding delay to infinite games with quantitative winning conditions. In a delay game, one of the players may delay her moves to obtain a lookahead on her opponent's moves. We show that determining the winner of delay games with winning conditions given by parity automata with costs is EXPTIME-complete and that exponential bounded lookahead is both sufficient and in general necessary. Thus, although the parity condition with costs is a quantitative extension of the parity condition, our results show that adding costs does not increase the complexity of delay games with parity conditions. Furthermore, we study a new phenomenon that appears in quantitative delay games: lookahead can be traded for the quality of winning strategies and vice versa. We determine the extent of this tradeoff. In particular, even the smallest lookahead allows to improve the quality of an optimal strategy from the worst possible value to almost the smallest possible one. Thus, the benefit of introducing lookahead is twofold: not only does it allow the delaying player to win games she would lose without, but lookahead also allows her to improve the quality of her winning strategies in games she wins even without lookahead.

==> delayfreegames.tex <==
An arena~$\arena$ is a tuple~$(V, V_I, V_O, E)$, where $(V,E)$ is a finite directed graph without terminal vertices and $\{V_I, V_O\}$ is a partition of $V$ into the positions of Player~$I$ and Player~$O$. A parity game with costs~$\game = (\arena, \col, \cost)$ consists of an arena~$\arena$ with vertex set~$V$, a priority function~$\col \colon V \rightarrow \nats$, and a cost function~$\cost \colon E \rightarrow \set{\epsilon, \inc}$. A play~$\rho$ is an infinite sequence~$v_0 v_1 v_2 \cdots$ of vertices such that $(v_i, v_{i+1}) \in E$ for all $i$. A strategy for Player~$O$ is a map~$\sigma \colon V^*V_O \rightarrow V$ such that $(v_i, \sigma(v_0 \cdots v_i)) \in E$ for all $v_i \in V_O$. The strategy~$\sigma$ is positional, if $\sigma(wv) = \sigma(v)$ for all $wv \in V^*V_O$. Hence, we denote it as mapping from $V_O$ to V. A play~$v_0 v_1 v_2 \cdots $ is consistent with $\sigma$, if $v_{i+1} = \sigma(v_0 \cdots v_i)$ for every $i$ with $v_i \in V_O$. The strategy~$\sigma$ is winning from a vertex~$v \in V$, if every play~$v_0 v_1 v_2 \cdots $ with $v_0 = v$ that is consistent with $\sigma$ satisfies the parity condition with cost, i.e., $\limsup_{n\rightarrow \infty} \paritydist(v_0 v_1 v_2 \cdots ,n) $ is finite. Whether Player~$O$ wins a parity game with costs from a given initial vertex can be determined in time $\bigo(n^{p(k)})$ for some polynomial~$p$, where $n$ is the number of vertices and $k$ the number of colors of the game~\cite{FijalkowZimmermann14}. Furthermore, if Player~$O$ wins such a game from a given initial vertex, then also with a positional winning strategy. 

